Sparse VideoGen: Accelerating Video Diffusion Transformers with Spatial-Temporal Sparsity

Diffusion Transformers (DiTs) dominate video generation but their high computational cost severely limits real-world applicability, usually requiring tens of minutes to generate a few seconds of video even on high-performance GPUs. This inefficiency primarily arises from the quadratic computational complexity of 3D Full Attention with respect to the context length. In this paper, we propose a training-free framework termed Sparse VideoGen (SVG) that leverages the inherent sparsity in 3D Full Attention to boost inference efficiency. We reveal that the attention heads can be dynamically classified into two groups depending on distinct sparse patterns: (1) Spatial Head, where only spatially-related tokens within each frame dominate the attention output, and (2) Temporal Head, where only temporally-related tokens across different frames dominate. Based on this insight, SVG proposes an online profiling strategy to capture the dynamic sparse patterns and predicts the type of attention head. Combined with a novel hardware-efficient tensor layout transformation and customized kernel implementations, SVG achieves up to 2.28x and 2.33x end-to-end speedup on CogVideoX-v1.5 and HunyuanVideo, respectively, while preserving generation quality. Our code is open-sourced and is available at https://github.com/svg-project/Sparse-VideoGen

==> text/3_Preliminaries.tex <==
\section{Preliminaries}

\subsection{Diffusion Transformers}
% A Diffusion Transformer Model (DiT) comprises three key components: a text encoder, a variational autoencoder (VAE), and the transformer itself. 

Diffusion models typically consist of three main elements: a text encoder, a variational autoencoder (VAE), and a denoising model designed to iteratively handle noise within the latent space. Diffusion Transformers specifically employ a transformer model for the denoising task.  
During the sampling phase, the text encoder interprets textual inputs to generate conditioning embeddings, while the VAE reconstructs the generated latent representation into pixel space. 
The denoising process involves the model incrementally improving a noisy latent representation over a sequence of timesteps. 
In each step, video diffusion transformers utilize self-attention to identify dependencies both within individual frames and across multiple frames, and employ feed-forward layers to enhance the latents.
By repetitively executing these steps over all timesteps, video diffusion transformers convert the random noise latent into a coherent video. 

% These components are run once, whereas the transformer operates iteratively at every denoising timestep, comprising more than 99\% of the total computational cost.


% A Diffusion Transformer Model comprises three key components: a text encoder, a variational autoencoder (VAE), and the transformer itself. During the sampling process, the text encoder and VAE are invoked only once, while the transformer is called at every timestep. 
% Consequently, the text encoder and VAE account for less than 1\% of the total sampling time. 
% Therefore, in the following discussion, we focus exclusively on the transformer component.

% Diffusion models simulate visual generation through a sequence of iterative denoising steps. Typically, the diffusion process is divided into a thousand timesteps during the training phase and reduced to just a few dozen timesteps during the inference phase.


\subsection{Video Generation with 3D Full Attention}
Recent video diffusion models commonly adopt 3D full attention that integrates temporal and spatial attention into a unified framework. While this approach often delivers superior performance, it comes at the cost of significantly higher computational demands, particularly when the context length is extensive—such as in cases of long video sequences or high-resolution content. We denote the total context length as $S$, the length of the text prompt as $T$, the number of frame as $F$, and the token per frame as $C$. In 3D full Attention, we have 
\[ S = T + F \times C. \]
As we visualize in Figure~\ref{fig:attention proportion}, since the 3D full attention's compute time is quadratic to context length but linear layers' compute time is linear to it, attention takes most of the computation when the context length is longer than 20k. 

\begin{figure}[t]
    \centering
    \begin{minipage}[t]{\linewidth}
        \includegraphics[width=0.95\linewidth]
        {figure/AttentionPortionBarChartGray2.pdf}
        \caption{Time proportion of every component in DiT. Attention module's time proportion increases rapidly in long context setting. 
        }
        \label{fig:attention proportion}
    \end{minipage}
\end{figure}


==> text/7_Discussion.tex <==
\section{Discussion}

\subsection{Long-tail Quantization Error}

\subsection{Efficiency Breakdown}
